Self-Improvement in Language Models: The Sharpening Mechanism

Recent work in language modeling has raised the possibility of self-improvement, where a language models evaluates and refines its own generations to achieve higher performance without external feedback. It is impossible for this self-improvement to create information that is not already in the model, so why should we expect that this will lead to improved capabilities? We offer a new perspective on the capabilities of self-improvement through a lens we refer to as sharpening. Motivated by the observation that language models are often better at verifying response quality than they are at generating correct responses, we formalize self-improvement as using the model itself as a verifier during post-training in order to ``sharpen'' the model to one placing large mass on high-quality sequences, thereby amortizing the expensive inference-time computation of generating good sequences. We begin by introducing a new statistical framework for sharpening in which the learner aims to sharpen a pre-trained base policy via sample access, and establish fundamental limits. Then we analyze two natural families of self-improvement algorithms based on SFT and RLHF. We find that (i) the SFT-based approach is minimax optimal whenever the initial model has sufficient coverage, but (ii) the RLHF-based approach can improve over SFT-based self-improvement by leveraging online exploration, bypassing the need for coverage. Finally, we empirically validate the sharpening mechanism via inference-time and amortization experiments. We view these findings as a starting point toward a foundational understanding that can guide the design and evaluation of self-improvement algorithms.

==> scratch.tex <==

\dfc{
\begin{itemize}
\item Do we want to try to say anything about inference-time algos
  like MCTS in this paper?
\end{itemize}
}

\dfc{Questions:
  \begin{itemize}
  \item Criticisms:
    \begin{itemize}
    \item It's also reasonable/practical to consider forms of
      self-improvement that leverage external signal (e.g., XPO), and this
      may be more useful in many settings.
      \begin{itemize}
      \item We can argue that this is complementary, since any method
        that uses external feedback can potentially be pushed a little
        further by pure self-improvement.
      \end{itemize}
    \item 
    \end{itemize}
  \item What is the distinction between self-training and
    self-improvement?
    \begin{itemize}
    \item Self-training: Any time we train a model on its own outputs
    \item Self-improvement: Broader problem. A tentative proposal: We
      have some task/objective/metric in mind, but we want to improve
      the performance of our model on this task without giving it any
      explicit feedback
      \item Another term we can use: ``Training-time
        self-improvement'' (to contrast with inference-time self-improvement).
    \end{itemize}
  \item 
    Positioning our work:
  \begin{itemize}
  \item How to distinguish from, e.g, \bestofn with a reward model?
    \begin{itemize}
    \item We are explicitly considering \emph{self-supervised}
      algorithms that do not require external feedback?
    \end{itemize}
  \end{itemize}
  \item Formal definition of \emph{sharpening}?
    \begin{itemize}
    \item Tilting policy $\pi$ towards its argmax?
    \end{itemize}
  \end{itemize}
  }
  \subsection*{Notation}
  \dfc{
 \begin{itemize}
 \item Base policy: $\piref$, other options include
   $\pi_{\texttt{base}}$ or $\pi_{\texttt{init}}$
   \begin{itemize}
   \item $\pi_{\texttt{base}}$ 
   \item Don't introduce $\pistar$ in general notation.
   \end{itemize}
 \item Use superscript for $\star$ ala $\ystar$, $\Cstar$
   \begin{itemize}
   \item Superscript
   \end{itemize}
 \item Examples: $x\ind{i}$ or $x_i$?
   \begin{itemize}
   \item Subscript
   \end{itemize}
 \item Responses are $y\in\cY$, autoregressive is special case where
   $\cY=\cV^{H}$ (vocabulary), $y=y_{1:H}$.
 \item Language modeling lingo:
   \begin{itemize}
   \item $\pi$ is a model
   \item $x$: prompt
   \item $y$: response
   \end{itemize}
 \item Notation: $(\eps,\delta,\gamma)$-sharpened policy:
 \[
         \bbP_{x\sim\rho}\brk*{\pihat\prn*{\Ygamma(x)}\geq{}1-\delta} \geq{} 1-\eps.
 \]
 Or do we want to do the version where $\eps$ and $\delta$ are pooled together?
 \item Failure probability: $\deltaf$. Or should we swap this w/
   $\delta$?
   \begin{itemize}
   \item Change context distribution to $\mu$, use $\rho$ for failure probability
   \end{itemize}
 \item $N$ as symbol for \bestofn / number of samples per context
 \item $n$ as number of contexts
   \item $m = n\cdot{}N$?
 \item $\Ygamma(x)=\crl*{y\mid{}
     \piref(y\mid{}x)\geq{}(1-\gamma)\piref(\ystar(x)\mid x)}$
 \item $\Ystar(x)=\Ygamma[0](x)$. Use this in place of $\ystar(x)$
   whenever we can (i.e., whenever a result does not require
   $\ystar(x)$) to be unique.
   \begin{itemize}
   \item Idea: Use $\mb{y}^{\star}_{\gamma}(x)$ and $\mb{y}^{\star}(x)$.
   \end{itemize}
 \item $\Cstar$ for $\En\brk*{\frac{1}{\piref(\Ystar(x)\mid{}x)}}$,
   $\Cstarg$ for $\En\brk*{\frac{1}{\piref(\Ygamma(x)\mid{}x)}}$
   \begin{itemize}
   \item $C_{\texttt{cov}}$, $C_{\texttt{cov},\gamma}$ (do this for
     now but macro it and see how the other looks once theorems are in place)
   \item $\texttt{Cov}$, $\texttt{Cov}_{\gamma}$
   \end{itemize}
 \item Conventions:
   \begin{itemize}
   \item Present main results with $\Ygamma$ if possible.
   \item Use $\Ystar(x)$ instead of $\ystar(x)$ is possible.
   \end{itemize}
 \end{itemize}
}



==> section_framework.tex <==




  












To understand why our sharpening objective is meaningful as a solution
concept for autoregressive language models, we observe
that when the response
$y=(y_1,\ldots,y_H)\in\cY=\cV^{H}$ is a sequence of tokens, our objective
\cref{eq:sharpening} sharpens
toward the \emph{sequence-level} arg-max response. Computing the
sequence-level arg-max for response for a language model, i.e.,
\begin{align}
  \label{eq:inference_time}
\argmax_{y_{1:H}}\piref(y_{1:H}\mid{}x)
\end{align}
is non-trivial and in general computationally intractable
\dfc{cite}. It is natural to imagine that sequence-level arg-max decoding might have
better performance on difficult reasoning tasks compared to more naive
decoding strategies such as \emph{greedy decoding} (which computes
$y_h=\argmax_{y_h\in\cV}\piref(y_h\mid{}y_{1:h-1},x)$) or beam search
\dfc{cite}. Our first result gives a stylized example where this is
indeed the case.
    \begin{example}[Benefits of sequence-level arg-max decoding]
      \label{ex:greedy}
      \dfc{Insufficiency of greedy decoding:
        \begin{itemize}
        \item First state simple/intuitive example with a couple actions/$H=2$.
        \item Then state more generic construction.
        \end{itemize}
      }
      \akcomment{Motivating example is when $\piref$ is a KL regularized optimal policy in some MDP. Then sampling from $\piref$ and greedy decoding might not be as good as MAP.}
    \end{example}

    \paragraph{Inference-time sharpening as a skyline}
Our discussion above highlights that inference-time computation
of the sequence-level arg-max response for $\piref$---or,
\emph{inference-time sharpening}---is a skyline for
the performance of any sharpening algorithm, and suggests that at
least in theory, this can lead to meaningful benefits. To validate
this empirically, we evaluate the performance of inference-time
sharpening for two stylized, yet challenging, reasoning tasks, \gametwentyfour \citep{yao2024tree} and
\stargraph \citep{bachmann2024pitfalls}.

Since exactly computing the sequence-level arg-max is intractable, we
implement inference-time sharpening by appealing to \BestofN sampling
\citet{stiennon2020learning,touvron2023llama,gao2023scaling,yang2024asymptotics}:
Given a prompt $x\in\cX$, we draw $N$ respones
$y_1,\ldots,y_n\sim\piref(\cdot\mid{}x)$, and return the response
$\yhat=\argmax_{y_i}\log\piref(y_i\mid{}x)$. The following proposition
shows that this scheme succeeds in computing an approximate arg-max
response whenever $\piref$ has sufficient coverage. To state the
result, let us define
$\Ystar(x)\ldef{}\argmax_{y\in\cY}\piref(y\mid{}x)$; we interpret
$\Ystar(x)\subset\cY$ as a set in order to accommodate non-unique
maximizers, but we will use the notation $\ystar(x)$ to indicate a
unique maximizer when it exists (i.e.,
$\Ystar(x)=\crl{\ystar(x)}$ in this case).
  \begin{proposition}[Inference-time \BestofN]
    \label{prop:bestofn_inference}
    Let a prompt $x\in\cX$ be given. For any $\deltafail\in(0,1)$ and $\gamma\in[0,1)$, as long as
    \begin{align}
      N \geq \frac{\log(\deltafail^{-1})}{\piref(\Ystar(x)\mid{}x)},
    \end{align}
    inference-time \BestofN sampling produces a response
    $
    \yhat \in \Ystar(x)$ with probability at least $1-\deltaf$.
  \end{proposition}

\paragraph{Empirical results}
  
  \cref{fig:validation} displays our findings for \gametwentyfour and
  \stargraph. We find that when $\piref$ is a pre-trained language
  model \dfc{details?}, inference-time \bestofn sampling with
  $\log\piref$ as the verifier leads to a
  meaningful increase in success probability for both tasks compared
  to greedy decoding and beam search. This suggests that sharpening is
  indeed a meaningful solution concept.


\dfc{Add footnote: If we say sharpening without qualification, we refer to training time}





    
    

    





    
            
    

    \paragraph{Training-time sharpening as amortized inference}

    Given the results above, we can view sharpening in the sense
    of our objective in \cref{eq:sharpening} as a form of
    \emph{amortized inference}. By expending extra
    computation at training time (through self-training), we aim to obtain a sharpened policy
    $\pihat$ that can compete with inference-time \BestofN sampling
    without having to expend inference-time computation.


    

\begin{remark}[Connection to maximum a-posteriori inference]
\dfc{Add references/explanation for connection to MAP/inference
  results in TCS here. Connect to diversity/diffusivity of the model
  a-la large language monkeys.}

\end{remark}


  


\section{Sharpening Algorithms for Self-Improvement}
\label{sec:algorithms}

  \dfc{
    \begin{itemize}
  \item In the remainder of the paper, we will analyze two natural
    algorithms for this task, \bestofnalg and \rlhfalg...
  \item Sketch here that asymptotically/with no errors, both algos
    converge to sharpened policy.
  \item What happens with errors/finite samples? What are the
    tradeoffs? In the remainder of
    the paper...
  \end{itemize}
}

\subsection{Self-Improvement through SFT: \bestofnalg}

\subsection{Self-Improvement through RLHF: \rlhfalg}


  


==> widebar.tex <==

\makeatletter
\let\save@mathaccent\mathaccent
\newcommand*\if@single[3]{%
  \setbox0\hbox{${\mathaccent"0362{#1}}^H$}%
  \setbox2\hbox{${\mathaccent"0362{\kern0pt#1}}^H$}%
  \ifdim\ht0=\ht2 #3\else #2\fi
  }
\newcommand*\rel@kern[1]{\kern#1\dimexpr\macc@kerna}
\newcommand*\widebar[1]{\@ifnextchar^{{\wide@bar{#1}{0}}}{\wide@bar{#1}{1}}}
\newcommand*\underbar[1]{\@ifnextchar_{{\under@bar{#1}{0}}}{\under@bar{#1}{1}}}
\newcommand*\wide@bar[2]{\if@single{#1}{\wide@bar@{#1}{#2}{1}}{\wide@bar@{#1}{#2}{2}}}
\newcommand*\under@bar[2]{\if@single{#1}{\under@bar@{#1}{#2}{1}}{\under@bar@{#1}{#2}{2}}}
\newcommand*\wide@bar@[3]{%
  \begingroup
  \def\mathaccent##1##2{%
    \let\mathaccent\save@mathaccent
    \if#32 \let\macc@nucleus\first@char \fi
    \setbox\z@\hbox{$\macc@style{\macc@nucleus}_{}$}%
    \setbox\tw@\hbox{$\macc@style{\macc@nucleus}{}_{}$}%
    \dimen@\wd\tw@
    \advance\dimen@-\wd\z@
    \divide\dimen@ 3
    \@tempdima\wd\tw@
    \advance\@tempdima-\scriptspace
    \divide\@tempdima 10
    \advance\dimen@-\@tempdima
    \ifdim\dimen@>\z@ \dimen@0pt\fi
    \rel@kern{0.6}\kern-\dimen@
    \if#31
      \overline{\rel@kern{-0.6}\kern\dimen@\macc@nucleus\rel@kern{0.4}\kern\dimen@}%
      \advance\dimen@0.4\dimexpr\macc@kerna
      \let\final@kern#2%
      \ifdim\dimen@<\z@ \let\final@kern1\fi
      \if\final@kern1 \kern-\dimen@\fi
    \else
      \overline{\rel@kern{-0.6}\kern\dimen@#1}%
    \fi
  }%
  \macc@depth\@ne
  \let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
  \mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}%
  \macc@set@skewchar\relax
  \let\mathaccentV\macc@nested@a
  \if#31
    \macc@nested@a\relax111{#1}%
  \else
    \def\gobble@till@marker##1\endmarker{}%
    \futurelet\first@char\gobble@till@marker#1\endmarker
    \ifcat\noexpand\first@char A\else
      \def\first@char{}%
    \fi
    \macc@nested@a\relax111{\first@char}%
  \fi
  \endgroup
}
\newcommand*\under@bar@[3]{%
  \begingroup
  \def\mathaccent##1##2{%
    \let\mathaccent\save@mathaccent
    \if#32 \let\macc@nucleus\first@char \fi
    \setbox\z@\hbox{$\macc@style{\macc@nucleus}_{}$}%
    \setbox\tw@\hbox{$\macc@style{\macc@nucleus}{}_{}$}%
    \dimen@\wd\tw@
    \advance\dimen@-\wd\z@
    \divide\dimen@ 3
    \@tempdima\wd\tw@
    \advance\@tempdima-\scriptspace
    \divide\@tempdima 10
    \advance\dimen@-\@tempdima
    \ifdim\dimen@>\z@ \dimen@0pt\fi
    \rel@kern{0.6}\kern-\dimen@
    \if#31
      \underline{\rel@kern{-0.6}\kern\dimen@\macc@nucleus\rel@kern{0.4}\kern\dimen@}%
      \advance\dimen@0.4\dimexpr\macc@kerna
      \let\final@kern#2%
      \ifdim\dimen@<\z@ \let\final@kern1\fi
      \if\final@kern1 \kern-\dimen@\fi
    \else
      \underline{\rel@kern{-0.6}\kern\dimen@#1}%
    \fi
  }%
  \macc@depth\@ne
  \let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
  \mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}%
  \macc@set@skewchar\relax
  \let\mathaccentV\macc@nested@a
  \if#31
    \macc@nested@a\relax111{#1}%
  \else
    \def\gobble@till@marker##1\endmarker{}%
    \futurelet\first@char\gobble@till@marker#1\endmarker
    \ifcat\noexpand\first@char A\else
      \def\first@char{}%
    \fi
    \macc@nested@a\relax111{\first@char}%
  \fi
  \endgroup
}
\makeatother


